Proof-of-Stake Longest Chain Protocols: Security vs Predictability

The Nakamoto longest chain protocol is remarkably simple and has been proven to provide security against any adversary with less than 50% of the total hashing power. Proof-of-stake (PoS) protocols are an energy efficient alternative; however existing protocols adopting Nakamoto's longest chain design achieve provable security only by allowing long-term predictability (which have serious security implications). In this paper, we prove that a natural longest chain PoS protocol with similar predictability as Nakamoto's PoW protocol can achieve security against any adversary with less than 1/(1+e) fraction of the total stake. Moreover we propose a new family of longest chain PoS protocols that achieve security against a 50% adversary, while only requiring short-term predictability. Our proofs present a new approach to analyzing the formal security of blockchains, based on a notion of adversary-proof convergence.

==> Nakamoto-PoS.tex <==

% =======================================
\section{Nakamoto-PoS Protocol Sketch}
\label{sec:nakamoto-pos}
The attempt to mimic Nakamoto protocol in PoS by \cite{fan2018scalable} is not secure (as demonstrated in \S\ref{sec:attack}); however the protocol with $g=0$ is still a very natural extension. We notice that while the balance attack was  demonstrably stronger than the private attack for all $g \geq 1$, it was not as effective for the  special case of $g=0$. It is possible that the $g$-greedy protocol is secure for $g=0$ and that $\beta_g = \frac{1}{1+e}$ is the true threshold of largest adversarial stake that can be tolerated. This remains an open question.

In this section we show that a subtle modification to the $0$-greedy protocol of \cite{fan2018scalable} can indeed be proved to be secure under a formal security model.  The $0$-greedy protocol of \cite{fan2018scalable} prescribes honest nodes to grow on {\em all} the longest chains of the block tree. In our subtly modified protocol we only grow on {\em one} of the longest chains (the chain which was seen the earliest); this is directly following the Nakamoto protocol where the mining process is conducted on only one of the leaves of the longest chains in the block tree. For this protocol, that we call Nakamoto-PoS, we show security in a standard security model (\S\ref{sec:model}) as long as the adversarial stake is no more than $\frac{1}{1+2e}$ (\S\ref{sec:analysis}). Although our suggested change to the basic $0$-greedy protocol appears subtle, this change  plays a currently  indispensable mathematical role in the security proofs in \S\ref{sec:analysis}.
When the honest nodes mine on  multiple longest chains simultaneously,
honest blocks can contribute to growing multiple chains. The adversary only needs to make sure that those chains are balanced as in the balance attack.

%\pv{please add one sentence to highlight this importance and why it might be playing a role}.
It remains open whether the $0$-greedy protocol of \cite{fan2018scalable} is secure and whether the true threshold of adversarial stake for security is $\frac{1}{1+e}$ (currently our mathematical techniques need the more conservative threshold of $\frac{1}{1+2e}$); these questions appear to be of significant mathematical depth and constitute an active research problem but outside the scope of this paper.


\cite{fan2018scalable} generalized the basic $0$-greedy protocol by changing the fork-choice rule (leading to the family of $g$-greedy protocols), but as we have seen in \S\ref{sec:attack}, this direction is inherently insecure. Instead, we generalize our basic Nakamoto-PoS protocol differently: we retain the fork choice rule, but change
the update of the randomness used in mining.
We describe this next, starting from
%We first present an informal sketch of our proposed Nakamoto-PoS  protoco, emphasizing the two main components: $c$-{\em correlation} and $s$-{\em truncation}.
%We present the protocol in full detail in Section~\ref{sec:protocols}.
%Our PoS protocol is designed from
first principles, starting with the Nakamoto longest chain rule.
A leader election (mining process) uses a general hash function of the form:
$    {\rm hash} = H({\rm header}).$
One option is to use
header $=$ ({\rm time}, \text{secret key}, {\rm parentBk}.{\rm hash}).
Including time ensures there is one leader election per time slot. The secret key links the hash to the owner of the stake. Including parentBk.hash provides  an unpredictable source of common randomness, which ensures that the outcome of the election can not be predicted in advance.
However, this allows the adversary to grind on the parentBk.hash, appending to all blocks in the block tree.
 This grinding attack is the same as the NaS attack and the growth rate of the private tree grown by an adversary  is amplified by a factor of $e$ (Appendix~\ref{app:nas}).

\begin{figure}[h]
%\begin{wrapfigure}{r}{.43\textwidth}
    \centering
\includegraphics[width=0.45\textwidth]{c_correlation_figure.png}
\caption{A snapshot of a block tree under $c$-correlation protocol with $c = 5$.
Each block has a header consisting of
header=(RandomSource of ParentBk, time).
The content of the block includes the public key of the coin (which we only denote by H or A in the figure), transactions, and the RandomSource of the block to be used in the next election. This random source is preserved from parent to children blocks, until one mines a block at height that is a multiple of $c$. In such a case, new RandomSource is drawn using the hash of the current header and the secret key of the miner. }
\label{fig:c-correction-protocol}
    \vspace{-0.5cm}
\end{figure}
%\end{wrapfigure}

In order to mitigate this grinding attack, we propose a principled approach by changing the source of randomness in mining: we call our scheme as
$c$-{\em correlated}-Nakamoto-PoS.
Let height of a block $b$ be the number of blocks in the chain
between the genesis and $b$ (including $b$ but not the genesis).
The height of the genesis block is zero.
Instead of updating the  source of randomness at every block with parentBk.hash,
we only update it at blocks of height multiples of $c$.
An example with $c=5$ is shown in Figure~\ref{fig:c-correction-protocol}.
The genesis block is initiated with a bit sequence to be used as a source of randomness denoted by a red triangle.
All of its descendant blocks
inherit the same bit sequence as a source of randomness, until it reaches height $c=5$.
This ensures that
for blocks at height less than $c$, even the adversarial blocks can only run one election at a time slot with the header (time, secret key,$\textcolor{red}{\blacktriangle}$).


Note that the content of the block is added after the leader election. Hence, the adversary can make multiple versions of the new block with the same header, but carrying different transactions and even appending to different parent blocks (as long as the parent block has a common source of randomness $\textcolor{red}{\blacktriangle}$. An example  is shown for two blocks with the header (time=4,secret key=A,$\textcolor{red}{\blacktriangle}$).


When the block chain reaches a height multiple of $c$, for example five in the figure, the block updates its source of randomness with the hash of the parent block.
This gives an opportunity  for the adversary to create multiple blocks at height five and grind on those multiple sources of randomness.
This correlation parameter $c$ gives the system designer the control to gracefully interpolate between full grinding attack with amplification factor $e$ (when $c=1$) and no grinding attack with amplification factor of one (when $c=\infty$).
One downside of having a large $c$ is that
it allows each node to predict further into the future when it will be elected a leader.
This opens new doors for attacks such as bribing, which is outside the security model studied in this paper. We discuss such external security threats in~\S\ref{sec:discuss}.





==> Related_works.tex <==
\section{Related works}
\begin{itemize}
    \item Ouroboros (Pramod) - Adv: Predictability and pre-bribing protection  + throughput advantage (try to point out that fruitchain may not be able to get high thruput)
    \item Algorand - Adv: Incentive compatibility, 1/3 vs 1/(1+e) for K = 1, but we allow K > 1 and can get closer to 1/2.
     Algorand has 1-round = r-step predictability , liveness vs consistency in the case of network partition / offline users. 
     competition vs cooperation (???).
     \item Dfinity: read Dahlia Malkhi's 5 page paper (supposedly get 1/2)
     https://eprint.iacr.org/2018/1153.pdf
     \item Snowwhite  read
    \item Tendermint PBFT (read)
    \item HotStuff and Sync Hotstuff
\end{itemize}

Main drawback: latency poor compared to BFT. We are tying our hands with no voting chains.

==> discussion.tex <==

\section{Discussion} \label{sec:discuss}

There are several attacks that are outside the scope of the security model studied in standard secure blockchain literature \cite{chen2016algorand,gilad2017algorand,yin2018hotstuff,bentov2016snow,kiayias2017ouroboros,david2018ouroboros,badertscher2018ouroboros,chronos}.
The design choices in a protocol inevitably trades off with such external attacks, but cannot be directly analyzed. This includes
nodes behaving rationally according to incentives,
eclipse attacks on network access, and bribing a node with external incentives.
Theoretical understanding of such attacks and securing against them requires different techniques than those studied in this paper, and we believe they provide interesting new  research directions.


%We discuss potential future research directions.

%\noindent
%{\bf Time and synchrony.} Our requirement on synchronized global clock could be relaxed with time synchronization sub-protocol proposed in  \cite{chronos}.

%Another  building block is $s$-truncated longest chain rule and $s$-delayed stake update. The parameter $s$ gracefully trades off security and adaptivity, i.e.~how fast the system adjusts to dynamically changing stakes. However, it is not known that an improved tradeoff can be achieved by another protocol. Characterizing the fundamental limit and designing new protocols to achieve this is of great interest for future research.


%Remainin issues:
%\begin{itemize}
%    \item It seems like  forward-secure signatures are not necessary for our security analysis, but is necessary for some orthogonal dimension of security (transactions). Do we still add them in this paper?
%    \item
%\end{itemize}


==> liveness.tex <==






==> old-lemma3.tex <==
Our goal is to get a bound on
$$q_{p,p+L} =P(\bigcap_{j= p}^{p+L} F_j^c).$$
This gives a bound on the tail of the distribution of the number of honest block arrivals for the next event $F_m$ to occur, starting at honest block $j$. This will be useful for proving persistence of the protocol.

\begin{lemma}
We have, under $e\lambda<1$, that 
\begin{equation}
q_{p,p+L} \leq A_1 \exp(-a_1 \sqrt{L})
\end{equation}
for some constants $A_1,a_1 > 0$ independent of $p$ and $L$. . 
\end{lemma}


\begin{proof}

Recall
\begin{equation}
    B_{ik} = \mbox{event that $D_i(\sum_{m = i}^{k-1} \mu_m) \ge  k - i-1$}
\end{equation}
Then 
\begin{equation}
    F_j^c = \bigcup_{(i,k): i < j, k >j} B_{ik}.
\end{equation}

Divide $[p, p+L]$ into sub-intervals of length $\sqrt{L}$. Introduce the atypical event:
\begin{equation}
    B = \bigcup_{(i,k): i \in [p,p+L] \mbox{~or~} k \in [p,p+L], i <k, k - i > 2 \sqrt{L}} B_{ik}
    \end{equation}
The event $B$ is the event that an adversarial tree catches up with a honest block far ahead.

By a union bound we have that $P(B) \leq Le^{-c \sqrt{L}}$.

Now look at even sub-intervals. Introduce the event that in the $\ell$-th even sub-interval
an adversarial tree that is at most in it or in the previous sub-interval catches up with a honest block at most $\sqrt{L}$ honest blocks ahead. 
Formally,
$$C_{\ell}=\bigcap_{j=p+ 2\ell \sqrt{L}}^{p+ (2\ell+1)\sqrt{L}-1}
\bigcup_{j - \sqrt{L} < i < j, j < k < j +\sqrt{L} } B_{ik}.$$
Note that for distinct $\ell$, the events $C_\ell$'s  are independent.
Also, we have
\begin{equation}
    \label{eq-qq}
    P(C_{\ell})\leq 1- p
    \end{equation}
%%    Indeed, we would have had equality in \eqref{eq-qq} if the union were over all $s$.
    
    Now, we have: 
    \begin{eqnarray}
    \label{eq-qqq}q &\leq& P(B) +P(\bigcap_{\ell=0}^{\sqrt{L}/2} C_{\ell})\\
    &=& \nonumber
    P(B)+(P(C_{\ell}))^{\sqrt{L}/2}\\
    &\leq& L e^{-c\sqrt{L}}+ (1-p)^{\frac{\sqrt{L}}{2}}
    \nonumber
    \end{eqnarray}
    where the equality is due to independence and the second inequality due to
    \eqref{eq-qq}.

Hence the theorem follows.
    
\end{proof}


==> old-static-analysis.tex <==
\section{Security analysis of the static stake protocol}
\label{sec:analysis}


Security of PoW systems, e.g. \cite{backbone}, rely on the fact that total number of blocks generated by the adversary under a PoW system grows linearly in time.
For a PoS system, the grinding attack allows the adversary to generate exponentially many blocks. However, one can hope to achieve security if the adversarial blocks added  in any single chain is still growing at most linearly.
We make this intuition precise in the following sections.

First, in Section~\ref{sec:private}, we
focus on a particular {\em private attack}, where the adversary privately grows a block tree with full grinding until it is long enough to take over the public block chain.
%We analyze a privately grown tree by an adversary with full grinding.
We provide a tight characterization of the growth rate of this tree, denoted by $\phi_c$, where $c\in{\mathbb Z}^+$ is a parameter of our choice in $c$-correlation.
%This shows that the adversary can add $\phi_c r f\Delta\beta$ blocks in $r$ rounds with a grinding attack, instead of $r f\Delta\beta$ blocks without grinding.
The adversary's mining power is effectively amplified by this factor of $\phi_c$.

This analysis provides a crucial building block in providing full security analysis for {\em any} adversary, in Section~\ref{sec:main}.
We show that the system is secure against all attacks allowed under our model in~\S\ref{sec:model}, as long as the adversary controls less than $1/(1+2\phi_c)$ proportion of the stake.
This includes
private chain attack,
grinding on the coin,
and grinding on the parent block, as well as
 an adversary that creates multiple copies of blocks with the same header, possibly appending to different parent blocks.

Throughout this section, we assume that $(i)$ the stake is not changing over time, $(ii)$ we use $s=\infty$ in $s$-truncation, $(iii)$ the slot duration is the same as the round duration, i.e.~$\delta=\Delta$, and use the terms slot and round interchangeably, and $(iv)$ $f$ is the expected arrival rate of a block per millisecond such that $f\Delta r$ blocks are generated in $r$ rounds on average. Note that when $s=\infty$, the $s$-truncation rule
is the same as the longest chain rule proposed by Nakamoto.


%Given the scope of the adversary, we need to appropriately restrict the environment (and the power of the adversary) to guarantee security. Consider the maximum total stake controlled by the corrupted nodes divided by the total stake that belongs to all  active (honest and corrupted) nodes at any  given slot. We denote this maximum adversarial fraction of the stake with $\beta$. We investigate security guarantees of Nakamoto-PoS as  functions of $\beta$, and the global parameters: the correlation parameter $c$ and security parameter $\kappa$. We further assume that the slot duration is the same as the round duration, i.e.~$\delta=\Delta$, and use the terms slot and round interchangeably.




% ========================================================================
\subsection{Analysis of the private Nothing-at-Stake attack}
\label{sec:private}


%The analysis crucially relies the intuition that although the corrupt nodes can generate far more blocks than honest nodes (as grinding on the common source of randomness is possible),  there cannot be too many adversarial blocks in a single chain of blocks. To make this intuition rigorous, we present necessary definitions and their probabilistic analyses.


%The analysis of typical execution crucially relies on Proposition~\ref{pro:adversarial}.

We analyze a particular attack, and the analysis will be used as  a fundamental building block to prove security of our protocol. Concretely, consider a private Nothing-at-Stake (NAS) attack, where an adversary grows a block tree in isolation. This private tree is hidden from the public view, until it is long enough to take over the public tree mined by the honest nodes.
This is the PoS counterpart of
the attack originally analyzed  by Nakamoto in \cite{bitcoin}.
The success of this attack depends on whether that private tree can grow faster than the public tree or not. We analyze how much stake the adversary needs to control in order to succeed. This threshold, denoted by $\beta_c$ below, increases with increasing $c$, i.e.~how long we keep the source of common randomness fixed in $c$-correlation. Eventually $\beta_c$ converges to $1/2$, recovering the security of private attack under PoW.


Under the $c$-correlation protocol, we define $(\phi_c,\psi_c)>0$ as the unique pair satisfying
\begin{eqnarray}
      F_c(\phi_c,\psi_c) & :=&  -\frac{1}{\phi_c}+1 + \psi_c + (1+\psi_c) \,\ln\Big(\frac{1}{\phi_c(1+\psi_c)}\Big) 
     +\frac{1}{c}\ln(1+c\psi_c) \nonumber\\
     &&\;\;\;\;+  \psi_c\,\ln\Big(1+\frac{1}{c\psi_c}\Big)\;=0\;, \text{ and } \label{eqn:relation1}\\
     \psi_c &=&\frac{c-c\phi_c+\sqrt{(c-c\phi_c)^2+4c\phi_c}}{2 c\phi_c}\;.   \label{eqn:relation2}
\end{eqnarray}

%$$\psi_c + \varepsilon(\psi_c - \frac{1}{4c\phi_c\sqrt{(c-c\phi_c)^2+4c\phi_c}})$$

Let $F_c(\phi):=F_c(\phi,\psi)$ with $\psi$ satisfying Eq.~\eqref{eqn:relation2}.
The uniqueness follows from the fact that $\nabla_{\phi}F_c(\phi)<0$ for all  $\phi>0$ as shown in Eq.~\eqref{eq:phiderivate}.
In the following theorem, we show that $\phi_c$ is an upper bound on the growth rate of the private tree, with a high probability.
$\psi_c$ does not have an immediate interpretation, and is an auxiliary variable that shows up in the proof of Proposition  \ref{lemma:discrete-chain-growth}, provided in Appendix~\ref{sec:discrete-chain-growth}.
\begin{propo}
\label{lemma:discrete-chain-growth}
Under the Nakamoto-PoS protocol with $c=O(1)$,
a private tree grown in isolation by an adversary with $\beta$ fraction of the stake for $r$ rounds starting from the genesis block
has a height upper bounded by $ \phi_c \beta f\Delta r (1 + \varepsilon)$ with a probability larger than $1-e^{- \Omega( \varepsilon \phi_c\beta f\Delta r )}$.
\end{propo}
\begin{table}[h]
\begin{center}
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c| }
 \hline
 $c$      & 1 & 2 & 3 & 4 & 5 & 6 &7&8&9 & 10\\ \hline
 $\phi_c$   & e & 2.22547  & 2.01030 & 1.88255  & 1.79545  & 1.73110 & 1.68103 & 1.64060 &1.60705 & 1.57860 \\
 \hline
 $\beta_c$ & $\frac{1}{1+e}$& 0.31003 & 0.33219 &0.34691 &0.35772 & 0.36615 & 0.37299 &
 0.37870 & 0.38358 & 0.38780
 \\ \hline
\end{tabular}
\end{center}
\caption{Numerically computed growth rate $\phi_c$ and stake threshold $\beta_c$.}
\vspace{-1cm}
\end{table}
Note that $\beta f\Delta r$ is the expected number of blocks generated by the adversary, if mining honestly without grinding. With grinding, this is amplified by a factor of $\phi_c$. With $c$-correlation, this amplification factor is reduced from $e$ when $c=1$ to $1$ when $c=\infty$.

When the private tree grows faster than the public tree, the adversary can eventually take over the entire block chain. This happens when $1-\beta<\beta \phi_c$, or equivalently $\beta>1/(1+\phi_c)$. We use $\beta_c:=1/(1+\phi_c)$ to denote this threshold on successful private NaS attack.
Note that in Theorem~\ref{thm:main}, $\beta<1/(1+2\phi_c)$ is required for security against a more powerful adversary who can also launch a hybrid of private and public attack.
For any given value of $c$, we can numerically compute the growth rate as shown in the table above.
This provides a guideline for a practitioner to choose the appropriate $c$-correlation, in order to achieve the desired level of security.
Note that $e\simeq2.71828$ is the base of the natural logarithm.
For a large enough $c$, the growth rate converges to one. The following analysis shows that the rate of convergence is  $1+\Theta(\sqrt{(\ln c)/c})$.
\begin{propo}
\label{lemma:discrete-chain-growth_upperbound}
For large $c$,
%\begin{eqnarray}
 $\phi_c  =  1+ \sqrt\frac{\ln c}{c}  + o\Big( \sqrt\frac{\ln c}{c} \Big)$, %\label{eq:aympphi}
%\end{eqnarray}
and
under the hypotheses of
Proposition~\ref{lemma:discrete-chain-growth}, the
height of the private tree is upper bounded by $ \phi_c \beta f\Delta r (1 + \varepsilon)$ with probability $1-e^{-\Omega(\varepsilon \phi_c \beta f \Delta r c^{-1} \sqrt{\ln c}\,)}$.
\end{propo}

\begin{figure}[h]
%\begin{wrapfigure}{l}{.3\textwidth}
    \centering
    %\includegraphics[width=0.4\textwidth]{log_k_2_avg_rate.jpg}
    \vspace{-.6cm}
\includegraphics[width=0.3\textwidth]{plot.png}
\put(-180,30){growth rate $\phi_c-1$}
\put(-100,-5){correlation parameter $c$}
    \caption{
    Theoretical prediction %from  Proposition~\ref{lemma:discrete-chain-growth}
     matches the simulated growth rate of the private NaS tree. %attack with $c$ correlation.% The asymptotic growth rate in Eq.~\eqref{eq:aympphi} closely
    }
    \label{fig:ccorrelation}
    \vspace{-.4cm}
%\end{wrapfigure}
\end{figure}
A proof is provided in Appendix~\ref{sec:proof_chaingrowth}. To show that this convergence rate is tight, we simulated the growth of a private tree with NaS attack under the optimal adversarial strategy given in Lemma \ref{prop:optimal_strategy_ccorrelation}.
In each round of our simulation, for every fixed block that is currently being mined on, its child-blocks are generated as a Poisson point process with rate $0.1$, i.e., $\beta f \Delta = 0.1$.
For each $c$, we ran the growth of the tree until the growth rate has sufficiently  converged, as shown in  Figure~\ref{fig:ccorrelation}. Each point is averaged over 10 independent runs.
We show the simulation results for $c\in\{2,4,8,16,32,64,128,256\}$ with corresponding  $\phi_c\in\{2.22547,1.88255,1.64060,
1.46780,1.34313,1.25244,1.18606  ,1.13725 \}$. We plot $\phi_c-1$ against $c$ in a log-log plot.
The red uses the numerically computed values of $\phi_c$, and
the blue line is the simulation result.
%the green line is the upper bound for $\phi_c$ given by Proposition \ref{lemma:discrete-chain-growth_upperbound}.
The gap between the red line and the blue line is due to the coarse discretization of the continuous differential equation in Eq.~\eqref{eqn:c-dep-growth-rate}, and can be made closer with a finer discretization and a longer run-time.
%In Figure \ref{fig:ccorrelation}, the red line and blue line are close showing that the numerical results are accurate.
%And three lines are parallel for large $c$, which indicates that the convergence rate in Proposition  \ref{lemma:discrete-chain-growth_upperbound} is tight.


% \subsection{Confirmation rule and desirable properties}





% ========================================
\subsection{Main results}
\label{sec:main}

We define a set of desirable
properties to prove security, introduced in \cite{backbone} for PoW systems.
Let $\mathcal{C}^{\lceil k}$ be the
chain resulting from pruning a chain $\mathcal{C}$ up to
$k$, by removing the last $k$ blocks at the end of the chain.
Note that $\mathcal{C}^{\lceil k}$ is a prefix of $\mathcal{C}$, which we denote by $\mathcal{C}^{\lceil k}\preceq \mathcal{C}$. The $k$-common prefix property ensures that after pruning a longest chain, it is a prefix of all future longest chains in the local view of any honest node.

\begin{definition}[$k$-common prefix]
We say a protocol and a corresponding confirmation rule have a {\em $k$-common prefix property}, if
any pair of longest chains $\mathcal{C}_1$ and
$\mathcal{C}_2$
in the view ${\sf VIEW}_{\Pi,\A,\Z}^{n,\cF}(\kappa)$ of any honest node $n$
at any two rounds $r_1 \leq r_2$, respectively, satisfy
$\mathcal{C}_1^{\lceil k} \preceq  \mathcal{C}_2 $.
    \label{def:prefix}
\end{definition}


In the absence of any adversary, each node will
contribute to the final ledger as many blocks as
their proportion of the stake. In the presence of an adversary, the chain quality property ensures that the contribution of the adversary is bounded.

\begin{definition}[$(\mu, \ell)$-chain quality]
We say a protocol and a corresponding confirmation rule have a  {\em $(\mu, \ell)$-chain quality property}, if
 in the view ${\sf VIEW}_{\Pi,\A,\Z}^{n,\cF}(\kappa)$ of
any honest node $n$ and at any round $r$,
the number of honest blocks
in any consecutive $\ell$ blocks of the longest chain is at least $\mu \ell$.
    \label{def:quality}
\end{definition}
Note that this requires chain quality to hold globally over all time.
In particular, this implies other chain quality conditions used in the analyses of
Ouroboros \cite{kiayias2017ouroboros} and Prism \cite{prism,li2019analysis}.
The chain growth property ensures that no matter
what the adversarial strategy is, the longest chain grows
at a certain rate.
\begin{definition}[$(\tau, s)$-chain growth]
We say a protocol and a corresponding confirmation rule have a {\em $(\tau, s)$-chain growth property},
if in the view ${\sf VIEW}_{\Pi,\A,\Z}^{n,\cF}(\kappa)$ of
any honest node $n$ and at any round $r$, $n$ adopts a longest chain $\mathcal{C}$, then it holds that after $s$ consecutive rounds $n$ adopts a chain that is at least $\tau s$ blocks longer than $\mathcal{C}$.
    \label{def:growth}
\end{definition}

When $\beta < 1/(1+2\phi_c)$, we show that these properties hold with high probability, under the following assumptions.

\begin{assumption}
    \label{asmp}
    For a choice of a correlation parameter $c\in{\mathbb Z^+}$, $\varepsilon>0$, and a  security parameter $\kappa>0$,
    \begin{itemize}
    \item the block arrival rate per slot is bounded by %$f\Delta = \omega((1/\kappa))$ and
    $f\Delta \leq {\varepsilon}/{2}$,
        \item
    we choose the total number of rounds of the system $r_{\rm max} = O({\rm poly}(\kappa))$ and $r_{\rm max} \geq 2\kappa/f \Delta $,
        \item the proportion of the adversarially controlled stake is upper bounded by $\beta \leq \left(\frac{1-\varepsilon}{1+2(1+\varepsilon)\phi_c}\right) $,
    \end{itemize}
    where $\phi_c\in[1,e]$ is the growth rate of a private tree that only depends on $c$ and is  defined in Section~\ref{sec:private}.
\end{assumption}

\begin{theorem}
    \label{thm:main}
    Under Assumption~\ref{asmp}, Nakamoto-PoS with a parameter $c\in{\mathbb Z}^+$ achieves
    \begin{itemize}
        \item
    $\kappa$-common prefix property in Definition~\ref{def:prefix},
        \item
    $\Big(\frac {(1-2\varepsilon)(1-\beta)}{4\phi_c},\kappa\Big)$-chain quality property
    in Definition~\ref{def:quality}, and
        \item  $\Big((1-\beta)(1-2\varepsilon)f\Delta,\frac{\kappa}{2 \phi_c f\Delta}\Big)$-chain growth property in Definition~\ref{def:growth},
    \end{itemize}
    with probability at least $1-e^{-\Omega(\varepsilon^2\, \kappa)}$.
\end{theorem}

We provide a sketch of the proof in Section~\ref{sec:sketch} and a complete proof in Appendix~\ref{sec:main_proof}.
Our goal is to generate a transaction ledger that satisfies
{\em persistence}  and {\em liveness} as defined in  \cite{backbone}.
Together, persistence and liveness guarantees robust transaction ledger; honest transactions will be adopted to the ledger and be immutable.  The formal definition of {\em persistence}  and {\em liveness} and how they follow from Theorem~\ref{thm:main} is derived in Appendix~\ref{sec:main_confirm}.





% ------------------
\subsection{Sketch of the proof of Theorem~\ref{thm:main}}
\label{sec:sketch}
%\pv{say a few lines about how this proof is different from the backbone paper and the subtleties involved.}

Our analysis technique builds upon
the security analysis of \bitcoin  backbone protocol in \cite{backbone}, with a crucial difference on how we bound the effect of the adversary on the blockchain.
The analysis of \bitcoin  backbone protocol
relies on the concentration of the total number of blocks an adversary can generate around its mean, $\beta f \Delta r$ blocks in $r$ rounds, with high probability.
For a PoS system, this is no longer true.
In $r$ rounds, an adversary can efficiently generate many, $e^{O(r)}$,
blocks with distinct headers.
If we include the multiple versions of the adversarial blocks with the same header, this number is unbounded.
This requires an innovation on how to measure the effectiveness of an adversary on tampering with the consensus of PoS blockchain protocols.
To this end, we propose
using the number of {\em in sequence} adversarial blocks as the measure of adversarial attack
as formally defined in Eq.~\eqref{eq:defV}.
Concretely, we build upon the growth rate of the branching process modeling private NaS tree from Section~\ref{sec:private} to show that the number of adversarial blocks added in a single chain in the entire block tree (including the private and public chains) in $r$ rounds is bounded by
$\phi_c \beta f \Delta r$.
This allows us to provide $k$-common prefix property, when $\beta$ is sufficiently small.

We define a {\em typical execution} (Definition~\ref{def:typical}), and show that this event happens with a large enough probability (Corollary~\ref{coro:typical}).
We complete a proof of Theorem~\ref{thm:main} in Appendix~\ref{sec:main_proof}, by showing that under the typical execution, the three desired properties hold.

%\subsubsection{Probabilistic analysis of the typical execution}
The analysis crucially relies the intuition that
although the
corrupt nodes can
generate far more blocks than honest nodes (as grinding on the common source of randomness is possible),
there cannot be too many
adversarial blocks in a single chain of blocks.
To make this intuition rigorous, we present necessary definitions and their probabilistic analyses.
%The analysis relies on the concentration of the number of blocks generated by honest nodes, and an upper limit on how many blocks can be included by corrupt nodes in a single chain.
For an interval $S$ of rounds, i.e.~$S=[r_1,r_2]=\{r_1,r_1+1,\ldots,r_2\}$ for some $r_1\leq r_2$, we define the following random variables.

%We follow \cite{backbone} in the definitions.

%\begin{definition}[$\beta$-corrupt property]
%A PoS system is said to be $\beta$-corrupt if at every round,  at least $1-\beta$ fraction of the stake is held by nodes who  follow the protocol honestly.
%\end{definition}

%Let $S$ be an interval of rounds. Let
\begin{itemize}
    \item $X[S]$ is the number of rounds in
    $S$ where
    one or more blocks
    are generated by honest nodes.
    \item $Y[S]$ is the number of rounds in
    $S$ where exactly
    one block
    is generated by honest nodes.
\end{itemize}
Under the model defined in~\S\ref{sec:model},
each honest node $n\in \N$
is elected with a probability
$\rho \times {\sf stake}_n/H_{\rm max}$
where $[0,H_{\rm max}]$ is the range of the pseudorandom number generated by VRF.
Assuming each node controls a  fraction of the stake bounded by  $O(1/|\N|)$, and for a large enough network size $|\N|$,
we approximate the number of blocks generated by the honest nodes in a single slot by a Poisson process ${\rm Poi}(f \Delta (\sum_{m\in \H}{\sf stake}_m)/(\sum_{m'\in \N}{\sf stake_{m'}}) )$,
where we define $f\triangleq \rho \times \sum_{m\in \N} {\sf stake}_m  /(H_{\rm max} \, \Delta)$
to be the block generation rate measured in blocks per milliseconds.
In practice, a target $f$ is chosen by the system designer and the ideal functionality provides the appropriate value of $\rho$ to the nodes in each slot. Further, note that this  {\em rate} of honest block generation  does not depend on the adversarial strategy.
The only thing that changes with the adversarial strategy is where those blocks append to.
This leads to the following concentration result implying that
enough unique honest blocks will be generated.
\begin{propo}
\label{pro:honest}
    Under any  adversary $\A$, the following inequalities hold with probability at least $1-e^{-\Omega(\varepsilon^2 f \Delta |S|)}$:
%    \begin{eqnarray}
    $|X[S]-\mathbb{E}X[S]| \le \varepsilon\mathbb{E}X[S] \;, \text{ and }
    |Y[S]-\mathbb{E}Y[S]| \le \varepsilon\mathbb{E}Y[S] .$
%    \end{eqnarray}
    Further, setting $f < 1/\Delta$ as is done in practical scenarios,  ${\mathbb E} X[S] \geq |S|(1- e^{-(1-\beta)f\Delta})$ and
    ${\mathbb E} Y[S] \geq (1-\beta)f\Delta\,|S| e^{-(1-\beta)f\Delta}$, where $\beta$ is the upper bound on adversarially controlled fraction of the stake, i.e.~$(\sum_{m\in \H}{\sf stake}_m)/(\sum_{m'\in \N}{\sf stake_{m'}})\geq 1-\beta $.
\end{propo}



We note that $X[S]$ and $Y[S]$ are the same
for the view of the honest nodes
and that of the adversarial nodes because they
depend only on the actions of the
honest nodes.
Every node keeps a history of all blocks
it sees on the blockchain.
Thus every node has a view of all
the blocks associated the blockchain
process in public. In addition, every node
has a view of blocks it mines in private.
We note that at the end of each round,
the views of the honest blocks synchronise (by
the model we assume)
and hence the honest blocks have a one unique
view at the start of a round.
We assume that there is a single adversary
who has access to the adversarial
strategy and adversarial blocks.
Hence the adversarial view is also unique.
Further, we note that every block in the
honest view is present in the adversarial view.
In addition, the adversarial view can include blocks
 mined by the adversary but
kept in private (and hence not present in the
honest view).

We define a block-tree $T_r$ as
the tree of blocks that are seen on
the blockchain process in the adversarial view
at the end of round $r$.

\begin{definition}[In-Sequence blocks]
Given a block-tree $T_r$ at the end of  round $r$,
we define a set of blocks $b_{i_1}, b_{i_2},
\cdots, b_{i_{\ell}}$ to be \textit{in sequence}
if on $T_r$,  $b_{i_{t}}$ is an
ancestor of $b_{i_{t+1}}$ for $t \in [\ell -1]$.
\end{definition}


Given a block tree in the
adversarial view at the end of
round $r$, $T_r$;
let $\mathcal{C}$ be the
longest public chain on it.
For $S = [r', r]$, an interval of rounds,
define $V[S]$ as the longest
sequence  of
\textit{in-sequence} blocks generated by the adversary
during rounds in $S$ on any chain
that diverged from $\mathcal{C}$
at round after $r'$ in $T_r$. More concretely,
\begin{align}
    V[[r',r]] &:= \max_{\substack{\mathcal{C}' \in T_r\\ \text{forking from }\mathcal{C} \\ \text{at round after }r' }} Z_{\mathcal{C}'}[[r',r]],
    \label{eq:defV}
\end{align}
where $Z_{\mathcal{C}}[S]$ is the number
of adversarially mined blocks on
a chain $\mathcal{C}$ in interval $S$
in the adversarial view at some round
after the largest round in $S$.
By forking we mean that a block in the
block tree has multiple successors.
This may occur either due to multiple honest
nodes obtaining blocks in a round or
due to one or more adversarially generated blocks.


\begin{propo}
\label{pro:adversarial}
 With probability at least
$1 - e^{-\Omega(\varepsilon \beta f\Delta \lambda )}$, $V[[r',r]] \le (1+\varepsilon) \phi_c \beta f \Delta(r-r')$ for all $r' < r- \lambda$.
\end{propo}


We note that all of these need not
be released in rounds in $S$. Thus $V[S]$
is defined based on the view of the adversary,
and may not be seen by the honest nodes.
We next define the notion of \textit{typical execution}.
\begin{definition}[Typical execution]
\label{def:typical}
An execution is $(\varepsilon, \lambda)$-typical
for $\beta$-corrupt system,
for $\varepsilon \in (0,1)$
and an integer $\lambda$, % \ge \frac{2}{(1-\beta)f \Delta}$,
if, for a set of at least
$\lambda$ consecutive rounds, the following hold
for any interval of rounds $S$  of length
more than $\lambda$:
    $(a)$ $|X[S]-\mathbb{E}X[S]| \le \varepsilon\mathbb{E}X[S]$;
    $(b)$ $|Y[S]- \mathbb{E}Y[S]|\le \varepsilon\mathbb{E}Y[S]$; and
    $(c)$ $V[S] \le (1+\varepsilon) \phi_c \beta f\Delta |S|$.
\end{definition}
There are at most $r_{\rm max}^2$ choices of $S$, and the following corollary follows from union bound.
This corollary follows from Propositions~\ref{pro:honest} and \ref{pro:adversarial}.

\begin{corollary}
The Nakamoto-PoS protocol executes with ($\varepsilon,\lambda$)-\textit{typical
execution} with probability at least $1- r_{\rm max}^2 e^{-\Omega(\varepsilon^2 f \Delta \lambda )}$.
\label{coro:typical}
\end{corollary}

We will set $r_{\rm max} \leq {\rm poly}(\kappa)$ and
$f\Delta\lambda=\Theta(\kappa)$, such that typical execution holds with probability at least $1-e^{-\Omega(\varepsilon^2\kappa)}$.
In Appendix~\ref{sec:main_proof},
we show that the desired properties hold under this typical execution.




% ==========================================
%\section{Security analysis of the dynamic stake protocol} \label{sec:dynamic}

%The stake is dynamically being updated via transactions included in the blockchain. If the stakes take effect immediately, the system is vulnerable against an adversary grinding on the secrete key of the coin as discussed in \S\ref{sec:protocols}.  We propose a buffer of $s$ time slots when updating the stake. However, a long-range private attack is still possible. We show that the proposed $s$-truncation scheme that generalizes Nakamoto longest chain protocol is secure against any adversary under the typical execution.

%\begin{theorem}
 %   \label{thm:dynamic}
%    Under the dynamic stake setting, under the Assumption~\ref{asmp},     distributed nodes running Nakamoto-PoS protocol        with a choice of $s=2\kappa/(f\Delta)$     generates a transaction ledger satisfying {\em persistence} and {\em liveness} in  Definition~\ref{def:public_ledger} with probability at least $1-e^{-\Omega(\varepsilon^2 \kappa)}$.
%\end{theorem}


%\noindent{\bf Proof sketch.} We prove it in three steps. First, we show that with static stake setting, common prefix, chain growth, and chain quality properties still hold for $s$-truncation protocol with $s=2\kappa/(f\Delta)$.Second, we show that with dynamic stake setting, the adversary can mine a denser private chain in consecutive $s$ time slots than public main chain only with a negligible probability.Last, we show that with dynamic stake setting and the stake update delay being $s$ time slots, any consecutive blocks of the main chain mined in $s$ time slots cannot be all adversarial under the $(\varepsilon,\lambda)$-typical execution.


%\begin{lemma}
%    \label{lem:longrange}
%\end{lemma}

% ==========================================

==> proofs-old-Section5.tex <==

We provide proofs of technical results.

% ================================================================
\subsection{Proof of Theorem~\ref{thm:main}}
\label{sec:main_proof}

We provide proofs of each of the three properties.


\subsubsection{Common prefix}

Given Corollary~\ref{coro:typical},
it suffices to prove that under the ($\varepsilon,\lambda$)-typical execution, the $\kappa$-common prefix holds, where $\kappa = 2 \phi_c f\Delta \lambda$.
Consider the discrete model where the
honest users successfully
generate $\text{Poi}((1-\beta)f \Delta)$ blocks
in a time slot
and the adversary has a probability of successfully
mining $\text{Poi}(\beta f \Delta)$.


\begin{lemma}
Suppose the block $b$  at height $k$ of a chain $\mathcal{C}$
was generated by an honest node in round $r$. Then
any block at height $k$ on any chain $\mathcal{C}'$
at any time is
either block $b$, one of the other blocks generated by some honest node
in round $r$, or is generated by the adversary.
\label{lemma:blk_height}
\end{lemma}
\begin{proof}
We show this by contradiction.

Let $\mathcal{B}_r$ be the set of honest blocks
computed in round $r$, and $\mathcal{B}_s$ be
the set of honest blocks computed in round $s$,
where $s > r$.

Let one of $\mathcal{B}_r$ be the $k$-th block
in chain $\mathcal{C}$. We have that each block
in $\mathcal{B}_r$ is in the $k$-th position in
some chain, because no honest miners would be mining
at chains which were at depth $k-2$.

For obtaining a contradiction assume that one of
the blocks of $\mathcal{B}_s$ is at the $k$-th position
of some chain $\mathcal{C}'$.

We note that  round $r+1$ on-wards, all honest miners mine
at position at least $k$ in any chain. This contradicts the
claim that some honest miner was mining at level
$k-1$ in some chain at round $s \ge r+1$, giving us the
result.
\end{proof}

\begin{remark}
We note that the this remark implies that
we have an injection between honest blocks  mined
in uniquely successful rounds which
are not on chain $\mathcal{C}$
to adversarial blocks on chain $\mathcal{C}$.
\end{remark}

% Let us now recall some notation as before.
% For an interval $S$ of rounds, let $Y[S]$
% be the number of rounds where the honest users
% were uniquely successful. Given a chain $\mathcal{C}$,
% let $Y_{\mathcal{C}}[S]$ be the number of blocks in
% the chain that were mined by honest users in
% uniquely successful rounds in $S$.


Similarly for a chain $\mathcal{C}$, recall that
$Z_{\mathcal{C}}[S]$ is defined to be the number of different rounds
in which adversary mines blocks on chain $\mathcal{C}$.
 Let us
focus on the block tree at round $r$, and the longest chain at
that round $r$ on the honest view
(if there are multiple longest chains pick any
one of them arbitrarily).
Define the following  events, with $r' = r-\lambda$, where $\lambda = \frac{\kappa}{2 \phi_c f\Delta}$. %{\bf{OR $\lambda = \frac{k}{2(1-\beta+e\beta)f\Delta}$?}}.

    \begin{align*}
        \tilde{E}_1[r',r] &=
        \bigcap_{0 \le \tilde{r} \le r'}\bigcap_{ \substack{\mathcal{C}\\ \text{diverges from} \\ \text{longest chain} \\ \text{at }\tilde{r}} }  \left\{
        \frac{1}{2}Y[\tilde{r},r] - Z_{\mathcal{C}}[\tilde{r}, r] > 0
        \right\} \\
        E_2 [r',r] &= \bigcap_{ \substack{\mathcal{C}\\ \text{diverges from} \\ \text{longest chain} \\ \text{at } r' }} \{ X[r',r] + Z_{\mathcal{C}}[r',r] < \kappa \}\\
        % E_3 [r-r', r] &= \{ X[r-r',r] > k/6 \}\\
        \tilde{E} [r',r] &=  \tilde{E}_1[r',r] \cap E_2 [r',r].
    \end{align*}


% \textbf{Define common prefix}
\begin{lemma}
Under the $(\varepsilon,\lambda)$-typical execution under a $\beta$-corrupt system with $f\Delta\leq\varepsilon/2$, and  $\beta < \left(\frac{1-\varepsilon}{1+2(1+2\varepsilon)\phi_c }\right)$,
the event
$\tilde{E}$ occurs for all $r$ and $r'=r-\kappa/(2\phi_cf\Delta)$.
\end{lemma}

\begin{proof}
We note that typical execution implies concentration
of $V[S]$ and hence concentration on all chains of
$\mathcal{C}$ diverging from $S$.
We further have concentration of $Y[S]$ and $X[S]$.


On the expected values, note that
$\mathbb{E}[Y[S]] = (1-\beta) f\Delta|S| e^{-(1-\beta)f\Delta}$,
then we have $Y[S] \geq (1-\varepsilon)\mathbb{E}[Y[S]] = (1-\varepsilon)(1-\beta) f\Delta|S| e^{-(1-\beta)f\Delta} > (1-\varepsilon)(1-\beta) f\Delta|S| e^{-f\Delta}$.
By definition, we have
$Z_{\mathcal{C}}[S] \le V[S] \le (1+\varepsilon) \phi_c \beta f\Delta|S|$.
The first condition gives us that
\begin{align*}
     \beta &< \frac{1-\varepsilon}{1 + 2(1+2\varepsilon)\phi_c },\\
    &\implies \frac{1}{2}(1-\varepsilon)(1-\beta) f\Delta|S|e^{-f\Delta} > (1+\varepsilon)\phi_c \beta f\Delta|S|,\\
    &\implies \frac{1}{2} Y[S] > V[S] \ge Z_{\mathcal{C}}[S]\;,
\end{align*}
where we assumed $f\Delta\leq \varepsilon/2$,
which gives us the occurrence of event $\tilde{E_1}$.
On the other hand, we have concentration of $X[S]$ and $Z_{\mathcal{C}}[S]$.
For $S=[r-\lambda, r]$, we have
\begin{align*}
    & X[r-\lambda,r]  \leq (1+\varepsilon)\mathbb{E}X[S] < (1+\varepsilon)(1-\beta)f\Delta \lambda,\\
    & Z_{\mathcal{C}}[r-\lambda,r]  \leq (1+\varepsilon)\phi_c  \beta f\Delta \lambda,  \\
\end{align*}
thus $X[r-\lambda,r] + Z_{\mathcal{C}}[r-\lambda,r] < (1+\varepsilon)(1-\beta + \phi_c \beta)f\Delta \lambda < 2(1-\beta+ \phi_c\beta)f\Delta \lambda < 2 \phi_c f\Delta \lambda = \kappa $,
which gives  the claim.
\end{proof}

\begin{lemma}
If $\tilde{E}[r', r]$ occurs with
$r' = r-\lambda = r-\frac{\kappa}{2 \phi_c f\Delta}$, the last $\kappa$ consecutive blocks of any chain $\mathcal{C}$ at round $r$ are mined in at least $\lambda$ consecutive rounds.
\label{lemma: eventE2}
\end{lemma}

\begin{proof}
By definition we know that $E_2[r',r] \supseteq \tilde{E}[r',r] $.
Event $E_2[r',r]$ implies that the total number of blocks of any chain $\mathcal{C}$ mined in interval $[r',r]$ is less than $\kappa$.
Therefore the $\kappa$-th deep block of $\mathcal{C}$ was mined on or before round $r'$.
\end{proof}

\begin{theorem}
If $\tilde{E}[r', r]$ occurs with
$r' = r-\frac{\kappa}{2 \phi_c f\Delta}$ for all $r$, the $\kappa$-common prefix property holds.
\end{theorem}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{CP_property.pdf}
  \caption{Round $r$ is the first round that the $\kappa$-deep prefix of the longest chain is changed.}
  \label{fig:cp_bb}
\end{figure}

\begin{proof}
Let $\mathcal{C}_1$ be a chain which is
the longest chain at current round $r_1$ and
$\mathcal{C}_2$ be a chain which is
the longest chain at a future round $r_2 > r_1$,
which violates the common-prefix property, i.e., $\mathcal{C}_1^{\lceil \kappa} \not\preceq \mathcal{C}_2$.


Let $r$ be the earliest round $r_1 \leq r \leq r_2$
such that there is a longest chain $\mathcal{C}_2'$ such
that $\mathcal{C}_1^{\lceil \kappa} \not\preceq \mathcal{C}_2'$.
If $r=r_1$,
define $\mathcal{C}_1'=\mathcal{C}_1$; otherwise, define
$\mathcal{C}_1'$
to be a longest chain at round $r - 1$.
Note that $\mathcal{C}_1^{\lceil \kappa}
\preceq \mathcal{C}_1'$.

Observe that by our assumptions such
an $r$ is well-defined (since e.g.,
$r_2$ is such a round, albeit not necessarily the smallest one);
refer to Figure \ref{fig:cp_bb} for an illustration.
Consider the last block $b^*$ on the common prefix of $\mathcal{C}_1'$
and $\mathcal{C}_2'$ that was mined by an honest node and
let $r^*$ be the round in which it was mined
(if no such block exists let $r^*= 0$).

Define the set of rounds $S = \{i : r^* < i \le r\}$.

Let $Y_{o}[S]$ be the number of blocks generated
in the interval
$S$ which are neither in $\mathcal{C}_1'$ or
$\mathcal{C}_2'$ by honest blocks in uniquely
successful rounds.
Using Lemma~\ref{lemma:blk_height}, we claim that,
\begin{align*}
    Y_{o}[S] + Y_{\mathcal{C}_1'}[S] & \le  Z_{\mathcal{C}_2'}[S],\\
    Y_{o}[S] + Y_{\mathcal{C}_2'}[S] & \le  Z_{\mathcal{C}_1'}[S],  \\
\end{align*}

We note that as at least one of $Y_{o}[S] + Y_{\mathcal{C}_1'}[S]$
and  $Y_{o}[S] + Y_{\mathcal{C}_2}'[S]$
has to be at least $\frac{1}{2}Y[S]$, we have
that
\begin{align*}
    \frac{1}{2}Y[S] \le \max \left( Z_{\mathcal{C}_1'}[S], Z_{\mathcal{C}_2'}[S]\right)
\end{align*}


However, we note that, $\tilde{E}[r_1-\lambda, r_1]$ holding gives us
$E_2[r_1-\lambda, r_1]$ holds, from Lemma \ref{lemma: eventE2}, which gives us that, the $\kappa$-th deep block of the chain $\mathcal{C}_1$
was mined on or before round $r_1 - \lambda$ and this implies $r^* < r_1 - \lambda \leq r - \lambda$.
Then we have
$\tilde{E}_1[r - \lambda, r]$ which gives us the a contradiction
and hence the claim.
\end{proof}

% ------------------------------------
\subsubsection{Chain quality}
We show this by contradiction.
Let $\mathcal{C}$ be the longest chain of an honest node at round $r$ and denote the $i$-th block of chain $\mathcal{C}$ as $b_i$ so that $\mathcal{C} = [b_1, b_2,\cdots,b_{\rm len(\mathcal{C})}]$.
Consider any $\kappa$ consecutive blocks in chain $\mathcal{C}$ denoted by $\mathcal{C}[u,v] := [b_u,\cdots,b_v]$.
Then let $N \geq \kappa$ to be the smallest number s.t. $N$ consecutive blocks $\mathcal{C}[u',v'] = [b_{u'}, \cdots, b_{v'}]$ include $\mathcal{C}[u,v]$ and have the properties:
(1) that the block $b_{u'}$ was mined by an honest node or is genesis in case such block does not exist, and (2) that there exists a round at which an honest node was trying to extend the chain ending at block $b_{v'}$.
Note that $\mathcal{C}[u',v']$ is well defined since $\mathcal{C}$ is such a chain.
Define $r_1$ as the round that block $b_{u'}$ was mined ($r_1 = 0$ if $b_{u'}$ is the genesis block), $r_2$ as the first round that an honest node attempts to extend $b_{v'}$.


Define the set of rounds $S = \{i : r_1 < i \le r_2\}$.
Let $H$ be the number of honest blocks on chain $\mathcal{C}$ mined in the interval $S$ and say $H < \mu \kappa$.
Then the number of blocks on chain $\mathcal{C}$ mined by adversary in the same interval $S$ is at least $N-1-H$, i.e., $Z_\mathcal{C}[r_1,r_2] \geq N-1-H$.
By chain growth property, we have $N-1 \geq X[r_1,r_2]$.
Adding them up, we have
\begin{equation}
    Z_\mathcal{C}[r_1,r_2] > X[r_1,r_2] - \mu \kappa.
    \label{eqn:chain_quality}
\end{equation}

We note that, $\tilde{E}[r_2-\lambda, r_2]$ holding gives us
$E_2[r_2-\lambda, r_2]$ holds, from Lemma \ref{lemma: eventE2}, which gives us that $b_u$,
was mined on or before round $r_2 - \lambda$.
Since block $b_{u'}$ was mined before block $b_u$, we have $r_1 \leq r_2 - \lambda$.
Then under the event $E_1[r_2-\lambda,r_2]$, we have
\begin{equation*}
     \frac{1}{2}Y[r_1,r_2] - Z_{\mathcal{C}}[r_1,r_2] > 0
\end{equation*}
Since  $X[r_1,r_2] \geq Y[r_1,r_2]$, we obtain
\begin{align*}
    X[r_1,r_2] - Z_\mathcal{C}[r_1,r_2] &> \frac{1}{2}Y[r_1,r_2] \\
      & \geq \frac{1}{2}(1-\varepsilon)\mathbb{E}[Y[S]]   \\
      & = \frac{1}{2}(1-\varepsilon)(1-\beta) f\Delta|S| e^{-(1-\beta)f\Delta} \\
      & \geq \frac{1}{2}(1-\varepsilon)(1-\beta) f\Delta \lambda e^{-f\Delta} \\
      & \geq \frac{(1-2\varepsilon)(1-\beta)}{4\phi_c}\kappa,
\end{align*}
which contradicts Equation \eqref{eqn:chain_quality} for $\mu =\frac {(1-2\varepsilon)(1-\beta)}{4\phi_c}$.
Therefore, in the interval $S$, at least $\mu \kappa$ blocks on $\mathcal{C}[b_{u'},b_{v'}]$ were mined by honest nodes and these blocks must be in $\mathcal{C}[u,v]$ by definition of $N$.

% ------------------------------------
\subsubsection{Chain growth}
Since honest nodes always work on the longest chain in the unique honest view, the length of the longest chain grows by at least $X[r-\lambda,r]$ in the interval $[r-\lambda,r]$.
And we have
\begin{equation*}
    X[r-\lambda,r] \geq (1-\varepsilon)\mathbb{E}[X[r-\lambda,r]] \geq (1-\varepsilon)\mathbb{E}[Y[r-\lambda,r]] > (1-2\varepsilon)(1-\beta) f\Delta \lambda,
\end{equation*}
which completes the proof.

% ------------------------------------
\subsection{Proof of Proposition~\ref{lemma:discrete-chain-growth}}
\label{sec:discrete-chain-growth}

The adversary is growing a private chain over the genesis block, under the $c$-correlation.
As illustrated in the figure below, the common source of randomness at a block
is only updated when the height is a multiple of $c$
(Algorithm~\ref{alg:PoS} line:\ref{algo:c-correlation}).
We refer to such a block $b$ with ${\rm height}(b)\%c = 0$ as
a {\em godfather-block}.
\begin{align*}
&{\rm RandSource}(b):= \nonumber\\ 
&\begin{cases}
\text{\sc VRFprove}\big({\rm RandSource}(\text{parent}(b)), {\rm time}, {\sf VRF}.sk(b)\big) , &\quad \text{if } {\rm height}\big(b\big)\%c=0,\\
{\rm RandSource}(\text{parent}(b)), &\quad \text{otherwise}
\end{cases}
\end{align*}
The randomness of a block changes only at \textit{godfather-blocks}. In other words, for $n\in\mathbb{Z}$, blocks along a chain at depths $\big\{nc, nc+1, nc+2,\cdots,nc+c-1\big\}$ share a common random number.
Two blocks are called {\em siblings-blocks} if they have the same parent block.
Given this shared randomness, the adversary now has a freedom to choose where to place the newly generated blocks. The next theorem provides a dominant strategy, that creates the fastest growing private tree.

\begin{lemma}
\label{prop:optimal_strategy_ccorrelation}
Under $c$-correlation,
the optimal adversarial strategy to grow the tree fast is to only fork at the parents of godfather-blocks. %Mining a sibling to a non-godfather-block does not increase the growth rate of the longest chain.
\end{lemma}
\begin{proof}
%We have seen that mining over multiple blocks in Esperanza does not effect the mining chances on a particular block.
Note that under the security model,
several types of grinding attacks are plausible.
First, at height multiple of $c$, the adversary can grind on the header of the parent of the godfather block, and run an independent election in every round.
Secondly, for blocks sharing the same source of randomness, once an adversary is elected a leader, it can generate multiple blocks of the same header but
appending on different blocks.
However, adding multiple blocks with the same header cannot
make the tree any higher than the optimal scheme.


\begin{figure}[h]
    \centering
    \includegraphics[width=.75\textwidth]{ctree}
    \caption{An example of $T^{(\Delta)}(t)$ with $c=5$ under the optimal strategy to grow the private NaS tree. Blocks forking from the same godfather-block share the same common source of randomness, as shown by the colors. To grow the tree fast, it is optimal to grow a single chain until the next godfather block. Circles with black outlines indicate blocks that are currently mined on.}
    \label{fig:my_label}
\end{figure}

Sibling non-godfather blocks share a common source of randomness and thus ‘‘mining events'' on these blocks are completely dependent.
Specifically, for sibling non-godfather blocks, there is only one leader election in each round.
As a result, for a particular non-godfather block $b$, the child-block of $b$'s any younger sibling (a sibling block mined after block $b$) should share the same header and identical source of randomness with one of $b$'s child-block.
Thus it is not necessary for a non-godfather block to have sibling blocks, that is, mining a sibling to a non-godfather block does not increase the growth rate of the longest chain in the adversarial block tree.
However, sibling god-father blocks have independent sources of randomness and thus mining multiple such block increase the growth rate of the longest chain.
\end{proof}






% In round $r$, the adversary follows the optimal strategy and independently mines on \textit{all} the blocks for new child-blocks.
From the point of view of a fixed block that is currently being mined on, its child-blocks are generated as a Poisson point process with
rate $\beta f \Delta$.
Let the number of blocks at height $\ell$ at time $t\in \{\Delta,2\Delta,\cdots\}$ be $X_\ell(t)$, and the expectation is
$x_\ell(t)=\mathbb{E}[X_\ell(t)]$. The genesis block is at heights zero.
Let $T^{(\Delta)}(t)$ denote the resulting random tree, and ${\rm height}(T^{(\Delta)}(t))$ denote the height of the tree.

Note that $\lim_{\Delta\to0}T^{(\Delta)}(t)$ converges to a continuous time process, where the block tree is growing with Poisson arrival rate of $\beta f$.
We denote this by $T^{(0)}(t)$.
Every block in current tree produces a child node arriving at rate $\beta f$ according to a Poisson arrival process.
This continuous time process dominates the discrete time process in the sense that
$\Pr( T^{(\Delta)}(t) \geq h) \leq \Pr( T^{(0)}(t) \geq h)$ for all $\Delta>0,h>0$ and $t>0$. As the growth of the height of the random tree is of our interest, we focus on the continuous time process in this section, and naturally extend the definitions of $X_\ell(t)$ and $x_\ell(t)$ to the continuous time counterparts.












We will first derive differential equations for $x_\ell(t)$.
Since the adversary only mines multiple godfather sibling blocks, the growth rate of blocks at level $i=nc+l$ (for $m,l\in\mathbb{Z},\; l < c$) depends on $i\%c=l$. In particular we have
\begin{equation}
\frac{dx_{nc+l}(t)}{dt}=\begin{cases}
\beta x_{nc+l-1}(t) & \qquad\text{for }l=0\\
\beta \big(x_{nc+l-1}(t) - x_{nc+l}(t)\big)&\qquad\text{for }l\in\{1,2,\cdots,c-1\}
\end{cases}\label{eqn:c-dep-growth-rate}
\end{equation}
with initial condition $x_{nc+l} = X_{nc+l}(0)=0$ and the root block satisfying
\[
x_{0}(t)=\mathbb{E}\big[X_{0}(t)\big]=\begin{cases}
1 & t\geq0\\
0 & t<0
\end{cases}.
\]
We solve for $x_{nc+l}(t)$ via Laplace transform. We first transform the differential equations \eqref{eqn:c-dep-growth-rate} in Laplace domain, obtain a closed form solution for $\hat{x}_{nc+l}(s)$. After that we transform the equations back to time domain.

First lets apply Laplace transform
for the above system of equations \eqref{eqn:c-dep-growth-rate}.
\begin{equation*}
s\hat{x}_{nc+l}(s)=\begin{cases}
\beta \hat{x}_{nc+l-1}(s) & \qquad\text{for }l=0\\
\beta \big(\hat{x}_{nc+l-1}(s) - \hat{x}_{nc+l}(s)\big)& \qquad\text{for }l\in\{1,2,\cdots, c-1\}
\end{cases}
\end{equation*}
Solving the above system of equations gives us
\[
\hat{x}_{nc}(s) = \frac{\beta^{n}}{s^{n+1}(1+s/\beta)^{(c-1)n}}.
\]
Let us substitute $\beta=1$ for simplicity.
We compute the inverse Laplace transform of $\hat{x}_{nc}(s)$ via convolution:
\begin{align}
    \hat{x}_{nc}(s)  &= \Big(\frac{1}{s^{n+1}}\Big)\Big(\frac{1}{(1+s)^{(c-1)n}}\Big)\nonumber\\
    x_{nc}(t) &= \mathcal{L}^{-1}\Big\{ \frac{1}{s^{n+1}}\Big\}\circledast\mathcal{L}^{-1}\Big\{ \frac{1}{(1+s)^{(c-1)n}}\Big\}\nonumber\\
            &= \Big( \frac{1}{n!}t^n\Big)\circledast\Big(\frac{1}{((c-1)n-1)!}e^{-t}t^{(c-1)n-1}\Big)\nonumber\\
            &= \frac{1}{n!((c-1)n-1)!}\int_{0}^{t}e^{u-t}(t-u)^{(c-1)n-1}u^ndu\nonumber\\
            & = \frac{e^{-t}}{(cn)!}\int_{0}^{t}e^{u}\frac{(cn)!}{n!((c-1)n-1)!}(t-u)^{(c-1)n-1}u^ndu\nonumber\\
            & \overset{(a)}{=} \frac{e^{-t}}{(cn)!}t^{cn}\int_{0}^{1}e^{tz}\frac{(cn)!}{n!((c-1)n-1)!}(1-z)^{(c-1)n-1}z^ndz\nonumber\\
            & = \frac{e^{-t}}{(cn)!}t^{cn}\mathbb{E}\Big[e^{tZ}\Big], \quad \text{where }  Z\in \text{Beta}(n+1 , (c-1)n) \nonumber\\
            &=\frac{e^{-t}}{(cn)!}t^{cn}\text{MGF}_{\text{beta}(n+1,(c-1)n)}(t)
            \label{eqn:mgf_equation}
\end{align}
The equality $(a)$ is obtained by change of variable $u=tz$. Our goal is to find the largest $\theta$ for which $x_{nc}(\theta n)$ decreases exponentially w.r.t $n$. Thus we evaluate the   $\text{MGF}_{\text{beta}(n+1,(c-1)n)}(t)$ at $t=\theta n$:
\begin{align}
    \text{MGF}_{\text{beta}(\alpha,\beta)}(t) &= 1+\sum_{p=1}^{\infty}\prod_{r=0}^{p-1}\Big(\frac{\alpha+r}{\alpha+\beta+r}\Big)\frac{t^p}{p!}\nonumber\\
    \text{MGF}_{\text{beta}(n+1,(c-1)n)}(t) &= 1+\sum_{p=1}^{\infty}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{t^p}{p!}\nonumber\\
    \text{MGF}_{\text{beta}(n+1,(c-1)n)}(\theta n) &= 1+\sum_{p=1}^{\infty}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!} \nonumber\\
     & \leq 1+\sum_{p=1}^{2e\theta n}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!} + \sum_{p=2e\theta n}^{\infty}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!}\nonumber\\
     & \overset{(a)}{\leq} 1+\sum_{p=1}^{2e\theta n}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!} + \sum_{p=2e\theta n}^{\infty}\frac{(\theta n)^p}{p!}\nonumber\\
     & \overset{}{\leq} 1+\sum_{p=1}^{2e\theta n}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!} + \sum_{p=2e\theta n}^{\infty}\frac{1}{2}^p\nonumber\\
     & \overset{}{\leq} 2+\sum_{p=1}^{2e\theta n}\prod_{r=0}^{p-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^p}{p!}
    \label{eqn:mgf_bound}
\end{align}

The summation in Equation \eqref{eqn:mgf_bound} is dominated by its largest term, which is given by
\begin{equation}
    \prod_{r=0}^{np_0-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^{np_0}}{np_0!} \label{eqn:mgf_largest}
\end{equation}where $p_0$ satisfies
\begin{align}
    &\frac{(1+p_0)}{(c+p_0)}\frac{\theta}{p_0} = 1 \label{eq:maximizer} \\
    \Longrightarrow &p_0  = \frac{\theta - c + \sqrt{(\theta-c)^2 + 4 \theta}}{2}, \label{eqn:p_0_solution}
\end{align}

Let $\phi_c = c/\theta$ and $\psi_c = p_0/c$, then Eq.~\eqref{eqn:p_0_solution} gives  Eq.~\eqref{eqn:relation2}.
Substituting Eq.~\eqref{eqn:mgf_bound} in Eq.~\eqref{eqn:mgf_equation}, we get %obtain that for large $n$
\begin{align}
    x_{nc}\big(\frac{nc}{\phi_c}\big) &\leq \frac{e^{-\frac{nc}{\phi_c}}}{(cn)!}{\big(\frac{nc}{\phi_c}\big)}^{cn}\Big(2+ (\frac{2ecn}{\phi_c})\frac{(n+nc\psi_c)! (cn)!}{n! (cn+nc\psi_c)!} \frac{\big(\frac{nc}{\phi_c}\big)^{nc\psi_c}}{(nc\psi_c)!} \Big)\nonumber \\
    & =  (\frac{2ecn}{\phi_c})e^{-\frac{nc}{\phi_c}}{\big(\frac{nc}{\phi_c}\big)}^{cn} \frac{(n+nc\psi_c)!}{n! (cn+nc\psi_c)!} \frac{\big(\frac{nc}{\phi_c}\big)^{nc\psi_c}}{(nc\psi_c)!} +2\frac{e^{-\frac{nc}{\phi_c}}}{(cn)!}{\big(\frac{nc}{\phi_c}\big)}^{cn} \nonumber \\
    & \leq (\frac{2ecn}{\phi_c})e^{-\frac{nc}{\phi_c}}{\big(\frac{nc}{\phi_c}\big)}^{cn} \frac{e(\sqrt{n+nc\psi_c})(\frac{n+nc\psi_c}{e})^{n+nc\psi_c}}{\sqrt{2\pi n}(\frac{n}{e})^n \sqrt{2 \pi (cn+nc\psi_c)}(\frac{cn+nc\psi_c}{e})^{cn+nc\psi_c}} \frac{\big(\frac{nc}{\phi_c}\big)^{nc\psi_c}}{\sqrt{2\pi nc\psi_c}(\frac{nc\psi_c}{e})^{nc\psi_c}} \nonumber\\
     &\;\;\;\;\;\;+ 2\frac{e^{-\frac{nc}{\phi_c}}}{\sqrt{2\pi cn}(\frac{nc}{e})^{nc}}{\big(\frac{nc}{\phi_c}\big)}^{cn} \nonumber \\
    & = \frac{e^2}{\phi_c \pi} \sqrt{\frac{1+c\psi_c}{2\pi(1+\psi_c)\psi_c}}e^{-\frac{nc}{\phi_c}+cn+nc\psi_c} \big( \frac{c}{\phi_c(c+c\psi_c)}\big)^{cn+nc\psi_c} \big(1 + \frac{1}{c\psi_c} \big)^{nc\psi_c} (1+c\psi_c)^n \nonumber\\
     &\;\;\;\;\;\;+ 2\frac{e^{-\frac{nc}{\phi_c}}}{\sqrt{2\pi cn}}{\big(\frac{e}{\phi_c}\big)}^{cn}\nonumber \\
    & = \frac{e^2}{\phi_c \pi} \sqrt{\frac{1+c\psi_c}{2\pi(1+\psi_c)\psi_c}} e^{nc\Big(-\frac{1}{\phi_c} + 1 + \psi_c + (1+\psi_c) \,\ln\big(\frac{1}{\phi_c(1+\psi_c)}\big) 
     +\frac{1}{c}\ln(1+c\psi_c) + \psi_c\ln\big(1+\frac{1}{c\psi_c}\big)\Big)} \nonumber\\
     &\;\;\;\;\;\;+ 2\frac{e^{-\frac{nc}{\phi_c}}}{\sqrt{2\pi cn}}{\big(\frac{e}{\phi_c}\big)}^{cn}\nonumber \\
    & = \frac{e^2}{\phi_c \pi} \sqrt{\frac{1+c\psi_c}{2\pi(1+\psi_c)\psi_c}} + \sqrt{\frac{2}{\pi cn}} e^{-nc(\frac{1}{\phi_c}-1+\ln(\phi_c))}\nonumber \\
    & = \frac{e^2}{\pi}\sqrt{\frac{c}{2\pi \phi_c}} + \sqrt{\frac{2}{\pi cn}} e^{-nc(\frac{1}{\phi_c}-1+\ln(\phi_c))}
\end{align}
The fixed point pair $(\phi_c,\psi_c)$ is the threshold above which the expected number of blocks at that level $h=cn=t\phi_c$ at time $t=cn/\phi_c$ starts to decrease exponentially.
Note that we always have $\frac{1}{\phi_c}-1+\ln(\phi_c)>0$ since $\phi_c>1$.
Notice that
\begin{eqnarray*}
    x_{nc}\Big(\frac{nc}{\phi}\Big) \;\;\leq\;\; \exp\{nc F_c(\phi) + O_n(1)\} \;,
\end{eqnarray*}
where $F_c(\phi):=F_c(\phi,\psi)$, and
$F_c(\phi,\psi)$ is defined in
 Eq.~\eqref{eqn:relation1}, and we plug-in $\psi = \psi(\phi)=({c-c\phi + \sqrt{(c-c\phi)^2+4c\phi}})/{2 c\phi}$ satisfying Eq.~\eqref{eqn:relation2}.
Next we show that the gradient of the exponent is strictly negative:

\begin{eqnarray}
    \frac{d F_c(\phi)}{d\phi} &=& \frac{1}{\phi^2} - \frac{1+\psi(\phi)}{\phi} + \frac{d\psi(\phi)}{d\phi} \frac{dF_c(\phi,\psi)}{d\psi} \nonumber \\
    &=& \frac{1-\phi-\sqrt{(1-\phi)^2+\frac{4\phi}{c}}}{2\phi^2}
    \;<\;0 \;,\label{eq:phiderivate}
\end{eqnarray}
for all $0<c<\infty$ and $\phi>0$, where we used the fact that
$d\psi(\phi)/d\phi= 0$ as $\psi(\phi)$ is the maximizer of
Eq.~\eqref{eqn:mgf_bound}.
Precisely,
${dF_c(\phi,\psi)}/{d\psi} = \ln((1+c\psi)/(c(1+\psi)\psi \phi))$.
This is zero, which follows from Eq.~\eqref{eq:maximizer}.
It follows that
\begin{eqnarray}
    x_{nc}\Big(\frac{nc}{\phi_c(1+\varepsilon)}\Big) \;\;\leq\;\; \exp\Big\{nc \varepsilon \frac{dF_c(\phi_c)}{d\phi} + O_n(1) + O_\varepsilon(n\varepsilon^2) \Big\} \;,
\end{eqnarray}
where we used the fact that $F_c(\phi_c)=0$ from the definition of $\phi_c$.
After re-scaling the time to take into account $f\Delta\beta$ blocks are generated per second (and letting $ nc=\phi_c r$), we get the desired result for any $c=\Theta(1)$.
If $c$ increases, the derivative in \eqref{eq:phiderivate} approaches zero.
A tighter analysis in this asymptotic regime
is provided in Proposition~\ref{lemma:discrete-chain-growth_upperbound} and in Appendix~\ref{sec:proof_chaingrowth}.

\subsection{Proof of Proposition~\ref{lemma:discrete-chain-growth_upperbound}}
\label{sec:proof_chaingrowth}

Let $\phi_c = 1+\varepsilon_c$, and suppose
$\varepsilon_c=o_c(1)$ and
$\psi_c=o_c(1)$ as $c$ grows.
From Eq.~\eqref{eqn:relation1}, Taylor expansion gives \begin{eqnarray}
F_c(\phi_c,\psi_c) &= -\frac12\varepsilon_c^2-\psi_c\varepsilon_c-\frac12\psi_c^2 + \frac{1}{c}\ln(1+c\psi_c) +\nonumber\\
     &\;\;\;\;\;\;\;\;\psi_c\ln(1+\frac{1}{c\psi_c}) + o_c(\varepsilon_c^2 + \psi_c^2)\;.
\end{eqnarray}
From Eq.~\eqref{eqn:relation2}, we know that
$\psi_c=O(\max\{1/(c\varepsilon_c),\sqrt{c}\})$.
Hence, in order for the dominating terms to cancel, we need $(1/2)\varepsilon_c^2 > (1/c)\ln(1+c\phi_c)$.
When $\varepsilon=\sqrt{(\ln c) / c} + o(\sqrt{(\ln c) / c})$ and the corresponding $\psi_c=O(1/\sqrt{c})$, then this can be satisfied for large enough $c$.
In this case, we get that $F_c(\phi_c,\psi_c) = - \Omega(\sqrt{\ln c}/c)$.


\iffalse
Let $c = \theta + \alpha c^{\frac{2}{3}}$, where $\alpha$ is to be chosen later.
Using this in Equation \eqref{eqn:p_0_solution}, we have
\begin{align}
    p_0 &= \frac{-\alpha c^{\frac{2}{3}} + \sqrt{\alpha^2 c^{\frac{4}{3}} + 4(c-\alpha c^{\frac{2}{3}})}}{2}  \nonumber \\
    & \leq \frac{c-\alpha c^{\frac{2}{3}}} {\alpha c^{\frac{2}{3}}} \nonumber \\
    & \leq \frac{1}{\alpha} c^{\frac{1}{3}}  \label{eqn:p_0_bound}
\end{align}
Using Equation \eqref{eqn:p_0_bound} in Equation  \eqref{eqn:mgf_bound}, we obtain
\begin{align}
    \text{MGF}(\theta n) &\leq 2e\theta n\prod_{r=0}^{np_0-1}\Big(\frac{n+r+1}{cn+r+1}\Big)\frac{(\theta n)^{np_0}}{np_0!}\nonumber\\
    & \leq 2e\theta n \Big(\frac{n+np_0}{cn+np_0}\Big)^{np_0}\frac{(\theta n)^{np_0}}{np_0!}\nonumber\\
    & \leq \frac{2e\theta n}{np_0!}(np_0)^{np_0}\nonumber\\
    & \leq 2e\theta ne^{np_0}\nonumber\\
    & \leq  2e\theta ne^{\frac{nc^{\frac{1}{3}}}{\alpha}} \label{eqn:mgf_upperbound}
\end{align}

Using Equation \eqref{eqn:mgf_upperbound} in Equation \eqref{eqn:mgf_equation} gives us
\begin{align}
    x_{nc}(\theta n) & \leq (2e\theta n)\frac{e^{-\theta n}}{(cn)!}(\theta n)^{cn}e^{\frac{nc^{\frac{1}{3}}}{\alpha}} \nonumber\\
       & \leq \Big(\frac{e\theta}{c}\Big)^{cn}e^{-\theta n+\frac{nc^{\frac{1}{3}}}{\alpha}} \nonumber \\
       & = \Bigg(\Big(\frac{e\theta}{c}\Big)^{c}e^{-\theta+\frac{c^{\frac{1}{3}}}{\alpha}}\Bigg)^n
\end{align}
Let $d=\theta/c = 1 - \alpha c^{-\frac{1}{3}}$, we now have
\begin{align}
     x_{cn}(dcn) & \leq \Big(\big(de\big)^{c}e^{-dc+\frac{c^{\frac{1}{3}}}{\alpha}} \Big)^n
     \label{eqn:expectation_upper_bound}
\end{align}
Thus $d$ has to satisfy
\begin{equation*}
\log(d) +1 - d + \frac{1}{\alpha}c^{-\frac{2}{3}}< 0,
\end{equation*}
for $x_{nc}(dcn)$ to decrease exponentially in $n$. This is achieved for $\alpha = \sqrt[3]{2}$, since by Taylor expansion, we have
\begin{align}
    \log(d) +1 - d + \frac{1}{\alpha}c^{-\frac{2}{3}} &< -\alpha c^{-\frac{1}{3}} - \frac{1}{2}\alpha^2 c^{-\frac{2}{3}} - \frac{1}{3}\alpha^3 c^{-1} + \alpha c^{-\frac{1}{3}}  + \frac{1}{\alpha}c^{-\frac{2}{3}}  \nonumber \\
    & = -\frac{2}{3c} < 0
    \label{eqn:taylor_expan}
\end{align}

Using Equation \eqref{eqn:taylor_expan} in Equation \eqref{eqn:expectation_upper_bound} gives us
\begin{align}
     x_{nc}(dcn) & \leq e^{-\frac{2n}{3}}
     \label{eqn:expectation_upper_bound1}
\end{align}
Define $D(t)$ as the maximum depth of the blocks at time $t$. Then by Markov inequality we have
\begin{equation}
    \mathbb{P}\big(D(dcn)\geq nc\big) = \mathbb{P}\big(X_{nc}(dcn)\neq 0\big) = \mathbb{P}\big(X_{nc}(dcn)\geq 1\big) \leq \mathbb{E}\big(X_{nc}(dcn)\big) < e^{-\frac{2n}{3}}
    \label{eqn:markov_inequ}
\end{equation}
Let $n=\frac{t}{dc}$ in Equation \eqref{eqn:markov_inequ}, we have
\begin{equation}
     \mathbb{P}\big(D(t)\geq \frac{1}{d}t\big) < e^{-\frac{2t}{3dc}}
\end{equation}

\begin{equation}
    \mathbb{P}\big(D(t)\geq (1+\epsilon)\frac{1}{d}t\big) \leq \mathbb{P}\big(D((1+\epsilon)t)\geq (1+\epsilon)\frac{1}{d}t\big)  <  e^{-\frac{2(1+\epsilon)t}{3dc}}
\end{equation}
\fi


\iffalse
\subsection{Proof of Lemma~\ref{lemma:discrete-chain-growth_FZ}}


The adversary is growing a private chain over the genesis block.
In round $r$, the adversary follows the optimal strategy and independently mines on \textit{all} the
blocks for new child-blocks.
From the point of view of a fixed block, its child-blocks are generated as a Poisson point process with
rate $\beta f \Delta$.
Let the depth of the tree denoted by $D[r]$
and defined as the maximum depth of its blocks at the end of round $r$.
Let the random variable $M_{i}[r]$ denote the number of blocks at depth $i$ (the genesis block is at depth $0$).

We first derive the expectation of $M_{i}[r]$.
$\mathbb{E}\big[M_{i+1}[r+1]\big]$ satisfies the following recurrence equation
\begin{equation}
\mathbb{E}\big[M_{i+1}[r+1]\big]=\mathbb{E}\big[M_{i+1}[r]\big]+\beta f \Delta \mathbb{E}\big[M_{i}[r]\big]\qquad\forall i\in\mathcal{I}\label{eq:discrete-growth-rate}
\end{equation}
with initial conditions $M_{i}[0]=0\;\forall\; i>0$. The genesis block satisfies
\begin{align}
M_{0}[r]=\mathbb{E}\big[M_{0}[r]\big]=\begin{cases}
1 & r \geq 0\\
0 & r < 0
\end{cases}. \label{eqn:initial_condition}
\end{align}
By induction and  Pascal's formula, it is easy to show that
\begin{align}
\mathbb{E}\big[M_{i}[r]\big]=\binom{r}{i} {(\beta f \Delta)}^i. \label{eqn:expectation_r_i}
\end{align}
From the above equation \eqref{eqn:expectation_r_i} we observe that the expected number of
blocks at a fixed depth $i$, grows with round $r$. On the other hand, for a fixed round $r$,
the expected number of blocks will become zero as the depth increases. Both these observations satisfy one's intuitions.


We will use equation \eqref{eqn:expectation_r_i} to derive the longest chain growth rate. For small $\epsilon>0$, let
\begin{equation}
i_{u}:=\big(1+\frac{\epsilon}{\sqrt{i_{u}}}\big)e \beta f \Delta r. \label{eqn:markov}
\end{equation}
Since $M_{i}[r]$ are positive random variable, applying Markov's
inequality gives us
\begin{align*}
\mathbb{P}\big(M_{i_{u}}[r] \neq 0 \big)\overset{(a)}{=}\mathbb{P}\big(M_{i_{u}}[r]\geq1\big) \leq\mathbb{E}\big[M_{i_{u}}[r]\big] & = \binom{r}{i_u} {(\beta f \Delta)}^{i_u}\\
 & <\frac{(\beta f \Delta r)^{i_{u}}}{i_{u}!}\\
 & \overset{(b)}{<}\big(1+\frac{\epsilon}{\sqrt{i_{u}}}\big)^{-i_{u}}\bigg(\frac{i_{u}}{e}\bigg)^{i_{u}}\frac{1}{i_{u}!}\\
 & \overset{(c)}{<}\big(1+\frac{\epsilon}{\sqrt{i_{u}}}\big){}^{-i_{u}}\frac{1}{\sqrt{2\pi i_{u}}}\\
 & \overset{(d)}{<} e^{-\epsilon\sqrt{i_{u}}}
\end{align*}
Equality (a) follows from the fact that $M_{i_{u}}[r]$ is an integer. Inequality (b) is obtained by substitution $\beta f \Delta r$ using equation \eqref{eqn:markov}. Inequality (c) uses Stirling's approximation.
Inequality (d) holds since $\big(1+\frac{1}{\sqrt{x}}\big)^x > e^{\sqrt{x}-1/2} $ for all $x>1$.

Let $\epsilon_1 = \frac{\epsilon}{\sqrt{i_u}}$, then we have
\begin{equation}
\mathbb{P}\big(D[r] < (1+\epsilon_1)e \beta f \Delta r \big)  = \mathbb{P}\big( M_{i_u}[r] = 0\big) \\
 > 1 -  e^{-\epsilon\sqrt{i_{u}}} \\
 = 1 -  e^{-\epsilon_1 i_u} \\
 > 1 -  e^{-\epsilon_1 e \beta f \Delta r},
\end{equation}
which concludes the proof.
\fi

\subsection{Proof of Proposition~\ref{pro:adversarial}}

Consider the block-tree at any
round in operation. Note that this block
tree depends upon both the honest operating
protocol which we have defined above
and adversarial strategy, which can be arbitrary.


Let $T_r$ be a block tree defined
according to the PoS protocol
conditioned
on the adversarial strategy.

Let $\mathcal{C}$
be a longest chain on $T_r$.

Define
\begin{align*}
    A_{\tilde{r}} = \{\mathcal{C}' \in T_r |  \mathcal{C}'
    \text{ diverged from } \mathcal{C} \text{ at round } \tilde{r}\}
\end{align*}

We note that in rounds $[\tilde{r},r]$, by Lemma \ref{lemma:discrete-chain-growth},
the growth of chains in $A_{\tilde{r}}$ would be
at most $\phi_c \beta f \Delta (r-\tilde{r}) (1+\epsilon_1)$
with probability at least $1 - e^{- \epsilon_1 \phi_c \beta f \Delta (r-\tilde{r})}$
if it were just an adversarial process.
However, considering the presence of honest nodes, we have that in rounds $[\tilde{r},r]$,
there are at most
$100 (1-\beta) f \Delta (r-\tilde{r}) \le 100(r-\tilde{r})$
honest blocks
generated with probability at least $1 - e^{-100 (1-\beta) \Delta f (r-\tilde{r})}$ by Chernoff bound for Poisson random variable.

Let $B_0$ be the last block
mined by honest nodes in rounds $[\tilde{r},r]$, which is at height $k_0$ and mined at round $r_0$.
By definition, all descendant blocks of $B_0$ are mined by adversarial nodes. If we contract the edge between $B_0$ and its parent block and move block $B_0$ right under the genesis block, then $V[\tilde{r},r]$ will not decrease and adversarial nodes can mine more blocks in rounds $[\tilde{r},r_0]$.
Repeat this operation for all honest nodes mined in rounds $[\tilde{r},r]$, we have that $V[\tilde{r},r]$
is upper bounded by the scenario where all $100(r-\tilde{r})$ honest blocks are right under the genesis block although this scenario violates rules for honest nodes.

Hence we have that the probability of a chain in $A_{\tilde{r}}$
having added more than
$\phi_c \beta f \Delta (r-\tilde{r}) (1+\epsilon_1)$
in-sequence adversarial blocks in $[\tilde{r},r]$ is at
most $100(r-\tilde{r}) e^{- \epsilon_1 \phi_c \beta f \Delta (r-\tilde{r})} + e^{-100 (1-\beta) \Delta f (r-\tilde{r})}$
for any $\epsilon_1 > 0$. In other words,
with probability,
1-$(r-\tilde{r}) e^{- \Omega(\epsilon_1 \phi_c \beta f \Delta (r-\tilde{r}))}$, we
have that
$V[\tilde{r},r] \le \phi_c \beta f \Delta (r-\tilde{r}) (1+\epsilon_1)$ for a given $\tilde{r}$.

Next we compute the probability that
for all $\hat{r} < r - \frac{k}{2 \phi_c f\Delta}$,
$V[\hat{r},r] \le \phi_c \beta f \Delta (r-\hat{r}) (1+\epsilon_1)$.
We do this by a union bound noting that,
the probability of failure is upper bounded by
\begin{align*}
    \sum_{\hat{r} = 0}^{r- \frac{k}{2 \phi_c f \Delta}} (r-\hat{r}) e^{- \Omega(\epsilon_1 \phi_c f \Delta \beta(r-\hat{r}))}
    &\le \sum_{\ell = \frac{k}{2 \phi_c f\Delta}}^{\infty} \ell e^{-\Omega(\epsilon_1 \phi_c f \Delta \beta\ell)},\\
    &= e^{- \Omega(\epsilon_1 \beta k)},
\end{align*}
giving us that with probability
$1 - e^{-\Omega(\epsilon_1 \beta k)}$, $V[[r',r]] \le (1+\epsilon_1)\phi_c \beta f \Delta(r-r')$ for all $r' < r- \frac{k}{2  \phi_c f \Delta}$.


\subsection{Proof of Theorem~\ref{thm:public_ledger}}
\label{sec:main_confirm}
\begin{definition}[from \cite{backbone}]
    \label{def:public_ledger}
    A protocol $\Pi$ maintains a robust public transaction ledger if it organizes the ledger as a blockchain of transactions and it satisfies the following two properties:
    \begin{itemize}
        \item (Persistence) Parameterized by $\kappa \in \mathbb{N}$, if in a certain round a transaction {\sf tx} appears in a block which is more than $\kappa$ blocks away from the end of the main chain of an honest node (such transaction will be called confirmed), then {\sf tx} will be confirmed by
        all honest nodes in the same position in the ledger.
        \item (Liveness) Parameterized by $u, \kappa \in \mathbb{N}$, if a transaction {\sf tx} is received by all honest nodes for more than $u$ rounds, then all honest nodes will report {\sf tx} at least $\kappa$ blocks away from the end of the ledger, i.e., {\sf tx} will be confirmed by all honest nodes.
    \end{itemize}
\end{definition}

The main result is that common prefix, chain quality, and chain growth imply that the transaction ledger satisfies  persistence and liveness.
\begin{theorem}
    \label{thm:public_ledger}
    Under Assumption~\ref{asmp}, distributed nodes running Nakamoto-PoS protocol
    generates a transaction ledger
    satisfying {\em persistence} and {\em liveness} in Definition~\ref{def:public_ledger} with probability at least $1-e^{-\Omega(\varepsilon^2 \kappa )}$.
\end{theorem}

\noindent {\bf Proof}. We first prove Persistence.
The proof is essentially based on the common prefix property of Nakamoto-PoS protocol.
\begin{lemma}[Persistence]
The public transaction ledger maintained by Nakamoto-PoS satisfies {\rm Persistence} parameterized by $\kappa$ with probability at least $1-e^{-\Omega(\varepsilon^2 \kappa )}$.
\end{lemma}
\begin{proof}
Let $\mathcal{C}_1$ be the main chain of an honest node $P_1$ at round $r_1$.
Suppose a transaction {\sf tx} is contained in $\mathcal{C}_1^{\lceil \kappa}$ at round $r_1$, i.e., it is confirmed by $P_1$.
Consider a main chain $\mathcal{C}_2$ of an honest node $P_2$ at a round $r_2 \geq r_1$.
By the common prefix property, $\mathcal{C}_1^{\lceil \kappa} \preceq  \mathcal{C}_2 $, which completes the proof.
\end{proof}

We next prove Liveness, which is based on the chain quality and chain growth property of Nakamoto-PoS protocol.
\begin{lemma}[Liveness]
The public transaction ledger maintained by Nakamoto-PoS satisfies {\rm Livenesss} parameterized by $u = \lceil \frac{2\kappa}{(1-\beta)(1-2\varepsilon)f\Delta} \rceil$ and $\kappa$ with probability at least $1-e^{-\Omega(\varepsilon^2 \kappa )}$.
\end{lemma}
\begin{proof}
We prove that after a transaction {\sf tx} is received by all honest nodes for at least $u$ rounds, then there exists an honest node with chain $\mathcal{C}$ such that $\mathcal{C}$ is the longest chain and {\sf tx} is included in $\mathcal{C}^{\lceil \kappa}$.
By chain growth property, the length of the main chain of any honest node has increased by at least $2\kappa$ blocks in consecutive $u$ rounds.

Then the chain quality property implies that at least one of the blocks in the $\kappa$ suffix of $\mathcal{C}^{\lceil \kappa}$ was mined by an honest node. Such a block would contain {\sf tx} since all honest nodes have received {\sf tx} as an unconfirmed transaction at that time.
Thus, the lemma follows.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:dynamic}}
\label{app:main_dynamic}
We first analysis $s$-truncation protocol under static stake setting.
With static stake setting, the adversary is not able to grind on any coin in public or in private, so Theorem~\ref{theo-tail} still holds.

Then let $t$ be the first time when one of the honest nodes (denoted as $P$) would make different decisions about what chain to work on based on $s$-truncation protocol and longest chain (LC) protocol.
In other words, all honest nodes equivalently follow LC protocol before time $t$.
Let the fork observed by $P$ at time $t$ be chain $\mathcal{C}_a$ and $\mathcal{C}_b$, which belong to two subtrees $\mathcal{T}_a$ and $\mathcal{T}_b$ respectively with last common block $b_{\rm fork}$ mined at time $t_{\rm fork}$.
Without loss of generality, assume that in the public view at time $t$, $\mathcal{C}_a$ is deeper than $\mathcal{C}_b$ while $\mathcal{C}_b$ is denser in the time interval with length $s$ after $b_{\rm fork}$, illustrated in Fig.~\ref{fig:s_proof}.

\begin{figure}[h]
    \centering
    \includegraphics[width=.75\textwidth]{s_truncation_proof.jpg}
    \caption{$t$ is the first time that the $s$-truncation protocol is applied by an honest node.}
    \label{fig:s_proof}
\end{figure}

Let the $s$-th block after $b_{\rm fork}$ on chain $\mathcal{C}_b$ be $b_1$ with height $\ell_1$ mined at time slot $r_1$.
Note that at time slot $r_1$, some of the blocks up to $b_1$ on chain $\mathcal{C}_b$ may be private but they will become public before time slot $r$.
Notice that the length of chain $\mathcal{C}_a$ at time slot $r_1$ must be less than or equal to $\ell_1$, otherwise it makes $\mathcal{C}_a$ denser than $\mathcal{C}_b$ then $\mathcal{C}_b$ won't be chosen at time slot $r$ according to our $s$-truncation protocol.
Let $r_2$ be the first time slot after $r_1$ such that chain $\mathcal{C}_a$ becomes the main chain according to LC protocol.
Note that $r_2$ is well defined since $r$ is such a time slot.

Let the public main chain at time slot $r_1$ be $\mathcal{C}^*$ with length $\ell^*$.
Case(i): $\ell^* \leq \ell_1$, then at some later time slot when length of the main chain grows to $\ell_1$, it must belong to $\mathcal{T}_b$, otherwise the fork will be longer than $\kappa$ blocks if the adversary makes chain $\mathcal{C}_b$ public. Then at time slot $r_2$, $\kappa$ common prefix property of LC protocol will be violated.
Case(ii): $\ell^* > \ell_1$, then $\mathcal{C}^*$ must belong to $\mathcal{T}_a$, otherwise $\mathcal{C}^*$ forks from $\mathcal{C}_a$ before or at block $b_{\rm fork}$, which would violate the $\kappa$ common prefix property of LC protocol at time slot $r_2$. Since honest nodes follow LC protocol in the interval $[r_1, r]$, only adversary will grow chain $\mathcal{C}_a$ before time slot $r_2$. One observation is that the length of $\mathcal{C}_a$ is dominated in distribution by the length of $\mathcal{C}_b$ in the interval $[r_1, r_2]$ since $\mathcal{C}_a$ is shorter than $\mathcal{C}_b$ at time slot $r_1$, so if the adversary can grow $\mathcal{C}_a$ to be the main chain, $\mathcal{C}_b$ will become even longer with a non-negligible probability, which violates $\kappa$ common prefix property of LC protocol


So far we have proved that with static setting, under typical execution, all honest nodes will actually follow LC protocol regardless the adversarial behavior, therefore common prefix, chain growth, and chain quality properties still hold for our $s$-truncation protocol with $s=\kappa$.

Next we consider the dynamic stake setting with $s$ stake update rule. In order to grind on the secrete key of a coin as discussed in \S\ref{sec:protocols}, the adversary must control $s$ consecutive blocks in the main chain.
Note that if the adversary starts grinding on some public adversarial blocks, that is the content of those blocks are changed, then this kind of grinding attack is equivalent to privately mine consecutive $s$ blocks since those public adversarial blocks have already been received by honest nodes.
However, the $\kappa$ common prefix property of LC protocol secures that the adversary cannot have a private chain denser than the main chain in consecutive $s$ blocks after the fork as we just proved.
If the adversary grinds on a private chain sparser than the main chain, the private chain won't be accepted by honest nodes in our $s$-truncation protocol.

Finally, the only way for the adversary to grind on a coin is controlling the last $s$ blocks in the main chain. However this is also excluded under typical execution since chain quality gives us that there must be at least one honest block in the last $\kappa$ blocks of the main chain, which concludes the proof.
